Atomicity and Abstraction for Cross-Blockchain Interactions

A blockchain facilitates secure and atomic transactions between mutually untrusting parties on that chain. Today, there are multiple blockchains with differing interfaces and security properties. Programming in this multi-blockchain world is hindered by the lack of general and convenient abstractions for cross-chain communication and computation. Current cross-chain communication bridges have varied and low-level interfaces, making it difficult to develop portable applications. Current methods for multi-chain atomic transactions are limited in scope to cryptocurrency swaps. This work addresses these issues. We first define a uniform, high-level interface for communication between chains. Building on this interface, we formulate a protocol that guarantees atomicity for general transactions whose operations may span several chains. We formulate and prove the desired correctness and security properties of these protocols. Our prototype implementation is built using the LayerZero cross-chain bridge. Experience with this implementation shows that the new abstractions considerably simplify the design and implementation of multi-chain transactions. Experimental evaluation with multi-chain swap transactions demonstrates performance comparable to that of custom-built implementations.

==> correctness.tex <==
\section{Correctness of the Atomic Protocol}
Given that a blockchain involves numerous participants, we operate under the assumption that communication between two blockchains will remain uninterrupted. This implies that once a message is dispatched, it will invariably reach its intended destination.

\subsection{Locking Mechanism Deadlock}
As we could see, our locking mechanism guarantees the correct sequential execution as long as all involved blockchains are locked and agree to take the next step. However, how to make sure that all blockchains are locked is the first thing we have to prove. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/lock.png}
    \caption{Two programs trying to lock interleaved state space}
    \label{fig:lock}
\end{figure}

Assume we have two multi-chain program $P_0$ and $P_1$, both working on chain $A$ and chain $B$. And the state space of $P_0$ and $P_1$ on both chains is interleaved, then only the program first locks both chain $A$ and chain $B$ can proceed. As shown in Fig.~\ref{fig:lock}.(a), $P_0$ locks both $A$ and $B$ before $P_1$, as a result, $P_0$ can proceed to execute while $P_1$ is aborted.
However, there's a dead-lock issue if the $P_0$ and $P_1$ locks different chains at the beginning and there is a race condition there. Shown in Fig.~\ref{fig:lock}.(b), the problem arises if $P_0$ locks $A$ and then tries to lock $B$ while $P_1$ locks $B$ and then tries to lock $A$, in current locking mechanism, both $P_0$ and $P_1$ will be aborted. Unlike traditional locking, which may create a deadlock, when two program will wait for the resources to be unlocked first. This locking mechanism is more safe for a transaction. Similar to the phone communication, if two people are keeping trying to call each other at the same time, then there will be no way for them to talk with each other.

Thus, in our correctness proof for an execution of a program, we assume that the program $P$ has successfully locked all the required state space. Any operation interleaved with the locked state space won't change it before the end of the program $P$ (unlocking with either updated or unchanged state space).

\subsection{Serializability and Linearizability}
First, we will prove the serializability and linearizability of the multi-chain program using our protocol.
\paragraph{Serializability} The serializability guarantees that the execution of multiple transactions, comprising numerous operations on one or multiple objects, is equivalent to some sequential (serial) execution of those transactions. In particular, it certifies that regardless of how the transactions interleave in practice, the end result appears as if the transactions were executed one after another, without overlap.
In the context of multi-chain applications, one transaction is divided into multiple operations across distinct blockchains, each involving a certain state space of each blockchain. When a transaction is under execution, it may interleave with other concurrent transactions. There are mainly two scenarios: 
\begin{itemize}
    \item {\bf Independent state space: } Some transactions might operate on a state space that's independent of the state space tapped by the current transaction. In such cases, these transactions don't interfere with the serializability of the ongoing transaction, as their operational domains don't overlap.
    \item {\bf Shared subset of state space: } There may be instances where another transaction targets a subset of the state space that the current transaction is manipulating. With the lock mechanism in place, only one of these conflicting transactions can advance at any given time. Consequently, the resultant execution trace will reveal that one transaction entirely precedes the other, ensuring no interleaved operations. The lock ensures that once a transaction begins execution on a shared state, other transactions are kept at bay until the former completes, preserving the essence of serializability.
\end{itemize}

\paragraph{Linearizability}
Linearizability focuses on ensuring that individual operations on single objects adhere to their real-time ordering. Essentially, it mandates that if one operation appears to execute before another in real-time, then it should also appear to execute before the latter in the system's history. This real-time guarantee ensures that any subsequent operation will only commence once the preceding operation concludes. 
In the context of our discussion, we aim to equip each multi-chain transaction with linear characteristics. To achieve this, we introduce a partial order to label the dependence relationship between different operations. This ensures that subsequent operations (with a higher order) can only execute once their preceding operations (with a lower order) have concluded over the entire state space.  In this way, we guarantee the linearizability of the execution process within the multi-chain program.

In conclusion, serializability ensures that the execution of a transaction remains isolated from other concurrent transactions, maintaining an equivalence to sequential execution. On the other hand, linearizability guarantees that the sequence of operations within a transaction strictly adheres to their predefined dependence relationships, reflecting their real-time order. Together, these guarantees uphold the integrity and order of operations in complex blockchain systems.

\subsection{Properties}
With serializability and linearizability, we can easily prove the other properties including two safety properties and a liveness properties.

the safety property involves the atomic consistency of the protocol. For any program $P$, the state update in each each should either be universally updated or remain unchanged. More specifically, it can be divided into two different properties based on different security scenario.
\begin{itemize}
    \item If the protocol terminates with a reported success, the state of all blockchains should be the state obtained by atomic execution of $EXECUTE(P)$. % TODO: define the atomic execution. %start point: maybe some global precondition for the execution of the program
    \item In the event of an anomaly in one blockchain or if a discrepancy in (simulated execution) arises in any chain, the state should remain unaltered.
\end{itemize}

Second, we still need a liveness property to guarantee the correct execution of the multi-chain program: If all blockchains reach a consensus on the multi-chain program, then the multi-chain program can always be executed to an end.

\subsection{Model Checking using TLA+}

Linearizability / Serializability

    .......S'...S|..x1 .. x2 .. x3....E|.........> 
behaves as if the action was executed instantaneously at some time between its start and end points. 
    ................S|x1x2x3E|.........> 


         |-----a----|
            |-----b------|
         ....a....b.......
         .......b.a......

         |----a-----|   |-------b-----|
         ....b .... a.... 


==> kedar-temporary.tex <==
We can consider a blockchain conceptually to be a deterministic state machine. 

  states S
  initial state i
  parameter domain X
  action set A . Each action a: S \times X \to S is a *partial* deterministic function. I.e., it may fail on some state, input combinations. 


In practice, we have 
	> multiple contracts each with its own state. So S is conceptually the cartesian product of the individual state sets
	> actions are partitioned amongst the contracts
	> each action only modifies a small part of the overall state. 

We ignore all these distinctions as they are irrelevant for the abstract presentation of the protocol and the correctness arguments. They are relevant for practical implementation. 


--------------------------------------

Distinct chains operate independently and concurrently. 


Say in the course of performing action a on chain C it is necessary to perform action b on distinct chain D. 

This cannot be done directly as part of the code of action a. That is because of the way the state machine is maintained by replication and consensus. The action a is performed many times by replicas of the state machine for C. Thus, in a direct call, every replicated execution of 'a' will invoke 'b', which is incorrect. 

Action b is issued only once. It may be performed multiple times by replicas on D. 

Instead, the invocation must be done indirectly.

1. Action a writes to chain C the intent to invoke b on chain D and suspends itself. 

2. An external "bridge" program B monitors chain C. It invokes b on chain D, obtains the result r, then "wakes up" action a with result r. 

3. Action a resumes with the result r. 


----------------------------------------

Now bridges are external to the chains and may be malicious. Thus, one cannot trust that (1) action b was actually performed on chain D; or (2) Even if b was performed, that the claimed result r is the actual result of performing b.

The 'Finality' condition on a bridge assures the property in one direction. This requires complex cryptography (eg zkbridge), but we'll abstract from that. 

We assume that Finality property of the bridge ensures the following: 

If bridge B claims that a certain transaction was performed on a chain, then this transaction was actually performed. (And this is verifiable independently.)


With these assumptions one can now prove for the remote-call protocol, that 

Theorem [remote call #1]: If action a on chain C invokes action b on chain D, then (1) b is performed on D at some later point in time, and (2) that the claimed result r is the actual result. 

more abstractly: 
Claim [remote call #2] If action a on chain C includes remote calls, the execution of 'a' proceeds as if all of the relevant chains were combined into one (??)

This is not true, as there is no cross-chain atomicity guarantee. 
 



==> major-points.tex <==
submit to FM track? 

Major points to make
	- programmer’s abstraction. Why necessary?
	- how implemented on bridges
	- what assumptions, how secure against malicious attacks and denial of service?
	>> especially stress role of trusted contracts
	   >> and say that trust in those contracts need not be *blind* — the contracts can come with proofs of correctness 
	- how differs from Herlihy et al work [theirs does not rely on bridges but is built bottom-up. Ours is easier to assemble and more general in scope]
	- experience: how easy is it to define transactions . Costs. How does the cost break down into components: actual transaction + enabling abstraction layer + bridge transmission. Knowing this one can focus future optimization efforts. 
	- what next? 

==> overflow.tex <==
\section{Introduction}

A blockchain system is a distributed ledger that maintains a continuously growing history of unalterable ordered information organized in a chain of blocks. As far, a wide range of blockchains based on different consensus protocols have been deployed. This diversity has precipitated a significant surge in the heterogeneity of the blockchain ecosystem. Looking forward, it is highly probable that we will see the emergence of a 'multi-chain universe'—a digital environment wherein disparate blockchain applications can seamlessly communicate, which is known as blockchain interoperability.

To assure secure and accurate interactions between distinct blockchains, numerous Cross-Chain Communication (CCC) protocols have been established. A fundamental feature of these protocols is the \emph{Finality Property}. This property requires the receiver blockchain to authenticate that a specific event has indeed been committed on the sender blockchain. %For instance, consider an application, App1, which commits to release 10 tokens on the receiver chain only once an equivalent number of original coins are locked on the sender chain. A lock message will be sent from the sender chain to the receiver chain for verifying it. 
%However, a situation may arise where Blockchain B fails to secure the 10 coins, but App1 erroneously perceives the coins as being locked. 
Without the finality property, the sender chain may create a fake message that is not committed on the sender chain. As a result, a user on the receiver chain would lose some property without a proper counter transaction on the sender chain, thereby reaping an unjustified benefit. 
%The 'Finality Property' within CCC protocols is designed to avert such discrepancies, thereby ensuring transactional integrity across varying blockchains.

Cross-Chain Communication (CCC) protocols can be categorised into two distinct types, namely ``trusted" and ``trustless", based on their varying trust assumptions and security models. Implementations of these protocols are commonly referred to as `cross-chain bridges'.
The ``trusted" CCC protocol introduces a third-party trust system, such as an Oracle network or a notary committee, to authenticate and verify the occurrence of specific events on an alternative chain. %It's fast, but insecure due to the centralized feature.
The ``trustless" CCC protocol, on the other hand, employs a `light client' approach, where one chain maintains an up-to-date version of the other's block-header. For instance, a light client of the sender chain would be implemented within the receiver chain. This method allows the receiver chain to acquire and update block header information from the sender chain, thereby verifying the occurrence of a specific event on the sender chain through Merkle proof method.
However, it should be noted that these CCC protocols primarily focus on the trust layer of the communication between two blockchains, aiming to maintain the \emph{Finality Property}. 
Conversely, there are other application-level blockchain interoperability protocols, such as cross-chain atomic swap facilitated by Hash Time-locked Contract (HTLC). However, these application-level protocols, which usually builds on top of the low-level bridges, are far more complicated to be designed and verified against the correctness.

%The overall flow for sending messages using LayerZero is as follows:
\begin{itemize}
    \item The user application will call \emph{send} function in the LayerZero endpoint to start the message transfer.
    \item The ultra light node will reward the assigned relayer, oracle and protocol provider (refund if extra fee is given) before emitting the Packet.
    \item The relayer picks up the packet and the related proof while the oracle provides the corresponding block header to the destination chain.
    \item The relayer will ask the ultra light client to verify the packet with the proof and call \emph{receive} function in the endpoint of the destination chain.
    \item The user application in the destination chain will pick up the packet and do something correspondingly.
\end{itemize}
There are two obvious problem in this process. One is the rewarding mechanism can result in many relayers doing nothing while still earning a lot of rewards. Though some fraud detection may prevent this happening, solving this in the protocol level is fundamental. The other problem is there lacks an acknowledgement process, which plays a very important role in ordered communication and safe remote contract execution in another chain.

\subsection{IBC in Cosmos}
%IBC seems to solve the above two problems that LayerZero has. After setting up the connection, channel and port, each node will be equipped with IBC module, which can send, verify and receive packets with the relayer network. There are two functions in IBC: \emph{sendPacket} and \emph{recvPacket}. The user application will first call \emph{sendPacket} to inform the IBC module to start the message transfer. A relayer will picks up the Packet and call \emph{recvPacket} in the destination chain to verify the packet and gain reward after emitting the packet. There are also special functions for acknowledgment. However, these acknowledgement functions may increase the complexity of relayer implementation. Note that relayer is trustless and anyone can be the relayer, and too much complexity in designing a relayer will make the whole process error-prone.

The CCC protocols are prone to security vulnerabilities and more than 2.5 billion dollars were hacked only in these bridges by the time we wrote the paper. % TODO: need a reference here
Though these bridges provide the required trust property in the implementation, the smart contracts based on the bridges are written manually, thus error-prone. In order to improve the security, many users and businesses tend to use bridge aggregaters, which expose several existing bridges in a single interface due to the similarity of elements among different CCC protocols, such as Multi-Message Aggregation (MMA). An alternative to bridge alternatives would be using security-enhancing mechanism by combining different sources of block-hash truth, as demonstrated in Gnosis Hashi. However, both methods operates at the implementation level, augmenting the security of the underlying bridges. Nevertheless, integrating these bridges securely into a smart contract remains a difficult task, since these bridge interfaces and communication processes are still too low-level for programming, not to mention the high-level multi-chain protocols. In current practice, if an application on one chain wants to communicate with other chains, the smart contract writers have to learn how to use different CCC protocols based on different blockchains they want to communicate with. This process is either unsafe and tedious.
 
%For example, the “dispatch” function in the Hyperlane CCC protocol, the “send” function in the LayerZero CCC protocol and “send\_packet” function in the IBC protocol have similar functionality for sending a message from one chain to another while different function names and different arguments are used in these protocols.
We believe that what is needed is an standard abstraction of CCC protocols for secure smart contract programming with the rapid development of the heterogeneity of the blockchain ecosystem. The abstraction can hide most of the details in the complicated CCC protocols and provide security guarantee during constructing the low-level CCC protocols from the abstracted protocol. On the other hand, with the standardization of the CCC protocols, the smart contract can be more portable, making the switch from one blockchain communication to another easier.
%the application writer will be able to write the smart contract more efficiently without knowing the details of the infrastructure for different protocols. However, it’s quite difficult to change all existing protocols’ interfaces to a standardized protocol because it requires a lot of engineering effort.

However, one problem will appear in the multi-chain program. Normally, the atomicity of the smart contract on the single chain is guaranteed by the consensus protocol of the blockchain. However, there is no consensus of the all the blockchains involved in a multi-chain program. How to ensure the atomicity among different chains remains a challenge.

\commentaj{Add bullet wise contributions of the paper?}

In this paper, we will demonstrate the design of BCCP (Bell-Lab Cross-Chain Protocol), a high-level abstraction for smart contract programming dealing with cross-chain communication. We implement an auto-translator to securely convert the standardized protocol into different CCC protocols based on the infrastructure of the specific chain. With this standardized protocol, application writers won’t need to worry about the detailed interface of different CCC protocols, which improve the scalability and operability a lot for designing the smart contract involving different CCC protocols. 
A development flow is shown in the figure: smart contract developers write a smart contract based on the standardized abstracted protocol without knowing the details how different bridges are implemented. Then, our tool can automatically translate the smart contract into a smart contract containing different CCC protocols based on the blockchain it wants to communicate with in a secure way.








%Further, we propose one novel feature in our protocol: traceability of transactions in multi-chain systems (since cross-chain communication requires the receiver chain to commit one transaction based on the sender chain status, a data structure to trace the dependence of the transactions of different blockchain is very important for security concerns). 
By using our standard protocol, we provide more security on top of the existing bridges. (we can come up with a formal property to analyze this traceability problem).

\subsection{Standardization of CCC protocols}
There is much current work ongoing to provide a standardized protocol for cross-chain communication. However, as noted here, these approaches are only promoting the strengths of their CCC protocol implementation (bridges) along with a standard proposal. While different bridges may have different pros and cons, it’s not yet to determine which one is the standardized protocol for all use cases. 
Another work, known as ERC-5164, proposes a uniform interface for EVM-based blockchain, it specifies how the message is dispatched on one chain and executed on the other chain in the interface. However, it can only be applied to EVM-based blockchain and focus on remote call of another chain. Our method further extends the idea and proposes more functionality such as atomic transaction in our protocol.

Instead of promoting a CCC protocol implementation, we propose an abstract layer of these protocols for the smart contract developers at the transport and application layer. The low-level bridges just need to provide a simple converter to our protocol to be integrated, which we think is the easiest way to let everyone agree on a standard protocol.


\knote{As of Dec 1, 2023}

\subsection{Single Blockchain Program Model}
A blockchain can be modeled as a state transition system with the following components:
\begin{eqnarray} 
  B &=& \langle S, W, S_0, T \rangle \text{, where} \nonumber\\
      &S& \text{: state space of the system} \nonumber \\
      &W& \text{: input space, the set of all possible inputs} \nonumber \\   
      &S_0& \text{: initial state space, } \nonumber \\
      &T& : S \times W \rightarrow S, T(s, w) = s' \nonumber \\
      &\text{ where}& \text{$s,s' \in S$ (current/next state), $w \in W$ (input)} \nonumber 
\end{eqnarray}

\hnote{For a group of smart contracts on chains to communicate with each other, we require certain assumptions on their
structure and behavior:
\begin{itemize}
    \item The contracts must support a mechanism that atomically creates a checkpoint of their state and locks the contract, preventing access by any entity other than the owner of the lock.
    \item If the contract is locked, any subsequent attempt to lock it or use it by an entity other than the lock owner must abort.
    \item It must be possible for a locked contract to roll back the contract state to the saved checkpoint or to update the state to a new value that is the result of an operation.
\end{itemize}
}

Specifically, for any $s_i \in S$, there are some attributes for it to have the lock mechanism:
\begin{itemize}
    \item {$locked$}: a Boolean value to indicate whether other programs are able to modify the $s_i$.
    \item  {$locked\_id$}: a Integer value recording the program working on it.
    \item {$locked\_val$}: as same type of $s_i$, indicating the execution value in the program. 
\end{itemize}
After adding the lock mechanism, as a result, we have three operations on the state variable: \emph{Lock, Update, Unlock} under a certain program with the identifier $id_P$. All these three operations are shown in the algorithm blocks.

For \emph{Lock} operation, the state will be locked for the current program (identified as $id_P$) while other programs have no way to modify the state until it is unlocked. For the current program $id_P$, it can only update the $locked\_val$ of the state when the state is locked. The details for update the state will be shown in the next operation \emph{Update}. Note that {\bf ACK} and {\bf ABORT} are used to notify the program of successful or failed progress, respectively. 
\begin{algorithm}
\caption{Lock the state $s$}
\begin{algorithmic}
\Procedure{Lock}{$s$, $id_P$}
    \If{$s.locked = false$}
        \State $s.locked := true;$
        \State $s.locked\_id := id_P;$
        \State $s.locked\_val := s;$
        \State {\bf ACK};
    \Else  { \bf ABORT};
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

In the \emph{Update} operation, the locking status of the state will be checked first. If it's not locked, then we can update the state as normal, otherwise, only the program that locked the state can modify the $locked\_val$ of the state and return a {\bf ACK} with the $order$ information of the operation (explained in the next section), while other programs must be terminated after {\bf ABORT}, waiting for the current program to finish.

\begin{algorithm}
\caption{Update the current state $s$}
\begin{algorithmic}
\Procedure{Update}{$s$, $w$, $id_P$, $T$}
    \If{$s.locked = false$} $s := T(s, w);$
    \ElsIf{$s.locked\_id = id_P$}
        \State $s.locked\_val := T(s.locked\_val, w);$
        \State {\bf ACK} $order$;
    \Else { \bf ABORT;}
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

\emph{Unlock} Operation may happen in two scenarios, one is successful execution of the program or at any failure point during the execution of the program. We use a $cond$ input to distinguish the two scenarios. If the program is successful, then the state will be updated with its $locked\_val$, else it should keep the previous state while unlocking the state. If the \emph{Unlock} operation is issued by other programs or on an unlocked state, then an {\bf EXCEPTION} will be raised.
\begin{algorithm}
\caption{Unlock the current state $s$}
\begin{algorithmic}
\Procedure{$Unlock$}{$s$, $id_P$, $cond$}
    \If{$s.locked = true \And s.locked\_id = id_P$}
        \State $s := cond ? s.locked\_val : s;$
        \State $s.locked := false;$
        \State {\bf ACK};
    \Else { \bf EXCEPTION;}
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

%updated state transition function $T'$ under a program with $id_P$ has the following property:
%\[
%\textbf{if } T_i(s_i, w_i) = s_i' \And s_i.locked == true 
%  \And s_i.locked\_id == id_P
%\]
%\[
%\textbf{then } T_i'(s_i, w_i) = s_i
%\]
%\[
%s_i.locked\_{val}' =  T_i(s_i.locked\_{val}, w_i),
%\]


\subsection{Decentralized Applications}
We can use a set of operations $\mathbb{T}$ to define a \hnote{general cross-chain transaction (CCT)} with an identifier $id_P$, where each $T \in \mathbb{T}$ represents an operation $T(s,w)$ in one blockchain. Note that each $T$ is executed in an atomic way in the corresponding blockchain, which is acknowledged by the consensus of the single blockchain. \hnote{These operations are related by an acyclic dependency (also called an ordering) relation that specifies which transactions depend on one another and how. For instance, it may be specified that operation a2 on chain c2 depends on operation a1 on chain c1; in that case, operation a2 can only be issued after a1 is complete (and successful). Operations that are not related by a dependency may be issued and performed in any order.} As a result, for each $T$, there are three attributes:
\begin{itemize}
    \item s: the state of the blockchain to be updated under $T$.
    \item w: the input that $T$ uses to update s. 
    \item chain\_id: it indicates where the operation will be executed the $T$.
    \item order: this value specifies at least how many operations are required to be executed before $T$ can be executed based on the dependency relationship. 
\end{itemize}

We assume that for all $T$s with the same order, are executed on different blockchains, and since there's no shared state space between two different chains, these $T$s are independent of each other. 

%All of the above attributes can be obtained either originally or from some graph computation based on the $G = (V, E)$.

Moreover, the multi-chain program should also contains the set of blockchains $\mathbb{B}$ involved in the program, as well as a set of the corresponding involved state space $\mathbb{S}$ in each chain.

As a result, the multi-chain program P can be defined as follows:
\[
P = (id_P, \mathbb{T}, \mathbb{B}, \mathbb{S}),
\]
and the execution is expected in the following:
\begin{algorithmic}
\Procedure{Execute}{$P$}
    \For {$i$}
        \For {each $T \in P.\mathbb{T} \And T.order = i$}
            \State $B := P.\mathbb{B}[T.chain\_id];$
            \State $s := P.\mathbb{S}[T.chain\_id];$
            \State $s := B.T(T.s, T.w);$
        \EndFor
    \EndFor
\EndProcedure
\end{algorithmic}
And we want this program to be executed in an atomic way: either happen or not happen at all to guarantee the consistency and security in the blockchain system. However, due to the decentralization of the blockchain system, it's challenging for atomicity, especially if one operation $T \in P.\mathbb{T}$ fails, we have to revert all other operations committed on other chains, which is generally not comprised to the immutability of the blockchain system. 

\subsection{Protocol Steps}
\hnote{
At a high level, our protocol follows the template of a two-phase commit protocol. Such protocols were originally developed for distributed database transactions which, however, operate under a different
model of trust and failure. Specifically, there are two roles in this protocol: the proposer and the participants, which is similar to the two-phase commit protocol. The proposer will broadcast the program P to obtain
all the agreements from participants with locking the current state, then ask the participants to execute each operation in the ‘Pending’ state and finally ask all the entities to unlock and update their state Overall, the protocol follows the steps below:
\begin{itemize}
    \item{\bf First Phase} The Proposer obtains agreement from all blockchains to “freeze” a portion of their state for executing the transaction. This is done by locking (and checkpointing) the state of all contracts on a blockchain that participate in operations that are part of this transaction. As the invocation of an operation may indirectly modify the state of multiple contracts, it is important that the “reach” of such modifications is known so that all affected state is locked. The reach can be determined by code inspection or through automated code analysis—we assume that it is done correctly.
    \item{\bf Second Phase} In the second phase, the proposer executes operations from the CCT in a sequence of rounds subject to two key properties: (a) the operations within a round must be independent of each other according to the acyclic ordering specified by the CCT and (b) for the k’th round R(k) and each operation f within R(k), the operations on which f depends (according to the CCT ordering relation) must have been successfully performed in rounds prior to the k’th round.
    \item {\bf Execution} The operations chosen in a round are executed on the individual blockchains. The locking mechanism allows the Proposer (but no other entity) to perform these operations.
    \item{\bf Abort} If an operation fails, the entire transaction is aborted, by restoring the state of every affected blockchain to its checkpointed original state before unlocking the blockchain for other operations.
    \item{\bf Success} If all operations succeed, the transaction is committed by updating the state of every affectedblockchain to its new state before unlocking the blockchain for other operations.
\end{itemize}

We will explain these steps in detail in the next section.
}

\subsection{Protocol Algorithm}
Due to the fair exchange theorem, a third part is required to guarantee the consistency that everyone does what others expect. But a centralized solution may introduce more vulnerability. As a result, we implement the two-phase commit protocol with a lock mechanism. The lock mechanism plays the role of the third party to anchor the behavior of all parties that agree to a certain program. Overall, the protocol is defined as follows:

%\begin{algorithm}
%\caption{Overall Protocol}
\begin{algorithmic}
\Procedure{Execute\_in\_MultiChain}{$P$}
    \For{each $B,S \in P.\mathbb{B}, P.\mathbb{S}$}
        \State $B$ check $P.\mathbb{T}$ and $P.id_P$
        \If{$B$ agrees} $B.Lock(S, P.id_P);$
        \Else { Abort;}
        \EndIf
    \EndFor
    \For {$i$}
        \For {each $T \in P.\mathbb{T} \And T.order = i$}
            \State $B := P.\mathbb{B}[T.chain\_id];$
            \If {$B$ agrees}
                \State $B.Update(T.s, T.w, id_P, T);$
            \Else
                \State $B.Unlock(S, id_P, false)$
            \EndIf
        \EndFor
    \EndFor
    \For{each $B,S \in P.\mathbb{B}, P.\mathbb{S}$}
        \State $B.Unlock(S, id_P, true)$
    \EndFor
\EndProcedure
\end{algorithmic}
%\end{algorithm}

Particularly, each blockchain is independent with each other, and the communication between each blockchain is achieved through the cross-chain bridges, which provide us the \emph{Secure Transfer} as the trust. We assume that the low-level bridges can guarantee to one blockchain that the counter-party blockchain did what he declared. And the lock mechanism is used to guarantee that another blockchain could only do what he claimed in the future. 

%Specifically, there are two roles in this protocol: the proposer and the participants, which is similar to the two-phase commit protocol. The proposer will broadcast the program $P$ to obtain all the agreements from participants with locking the current state, then ask the participants to execute each operation in the `Pending' state and finally ask all the entities to unlock and update their state. 
A sketch of the proposer design is shown below:

\begin{algorithm}
\caption{Proposer Design}
\begin{algorithmic}
\Procedure{Propose}{$P$} \Comment{Init}
    \For{each $B \in P.\mathbb{B}$}
        \State send $B, (P, Lock);$
    \EndFor
    %\State count = 0;
    \State goto Pending;
\EndProcedure

\Procedure{Progress}{$ACK$} \Comment{Pending}
    \If {receive $Lock\_ACK$ from all other chains}
        \For{each $T \in P.\mathbb{T} \And T.order = 0$}
            \State $B := P.\mathbb{B}[T.chain\_id]$;
            \State send $B, (T, P.id_P)$;
        \EndFor
    \EndIf
    \If {receive $Update\_ACK\_i$ from all other chains}
        \If{ $i$ is the last in $P$}
            \State goto Executed;
        \EndIf
        \For{each $T \in P.\mathbb{T} \And T.order = i+1$}
            \State $B := P.\mathbb{B}[T.chain\_id]$;
            \State send $B, (T, P.id_P)$;
        \EndFor
    \EndIf
\EndProcedure
    
\Procedure{Execute}{$P$} \Comment{Executed}    
    \For{each $B \in P.\mathbb{B}$}
        \State send $B, (P, Unlock, true)$
    \EndFor
    \State goto Init;
\EndProcedure

\end{algorithmic}
\end{algorithm}

This is a sketch of the participant design and it is passively executing all the messages from the proposer. Note that the proposer won't introduce a centralized problem since all participants can abort the whole program in any step before they do any update.
\begin{algorithm}
\caption{Participant Design}
\begin{algorithmic}
\Procedure{Receive}{$msg$}
    \If{$msg = (P, Lock)$}
        \State $Lock(S, P.id_P);$
    \ElsIf{$msg = (T, P.id_P)$}
        \State $Update(S, W, P.id_P, T);$
    \ElsIf{$msg = (P, Unlock, true)$}
        \State $Unlock(S, P.id_P, true)$
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}




==> result_highlights.tex <==
\subsection{Result Highlights}
This can be an optional section.

We can highlight the key results in here.

==> setup.tex <==
\subsection{Setup}
Describe the experimental set here. We need to put following things: capacity (CPU, MEM, Network BW etc.) of the the machines used in testbed and that assumed in the simulation

Details of trace-replay or artificial tranasactions being used for simulations

What is the benchmark for the testbed.

What are your baselines and explanation for why these baselines are comprehensive

==> simulation.tex <==
\subsection{Simulation Experiment Results}

We need to have some results either here or in the formal analysis corresponding to each major contribution of the paper.

-- Execution time of BCCP vs other Baseline protocols

\subsubsection{Parameter Sensitivity Analysis}

==> testbed.tex <==
\subsection{Testbed Experiment Results}
